CSFCube -- A Test Collection of Computer Science Research Articles for Faceted Query by Example

Query by Example is a well-known information retrieval task in which a document is chosen by the user as the search query and the goal is to retrieve relevant documents from a large collection. However, a document often covers multiple aspects of a topic. To address this scenario we introduce the task of faceted Query by Example in which users can also specify a finer grained aspect in addition to the input query document. We focus on the application of this task in scientific literature search. We envision models which are able to retrieve scientific papers analogous to a query scientific paper along specifically chosen rhetorical structure elements as one solution to this problem. In this work, the rhetorical structure elements, which we refer to as facets, indicate objectives, methods, or results of a scientific paper. We introduce and describe an expert annotated test collection to evaluate models trained to perform this task. Our test collection consists of a diverse set of 50 query documents in English, drawn from computational linguistics and machine learning venues. We carefully follow the annotation guideline used by TREC for depth-k pooling (k = 100 or 250) and the resulting data collection consists of graded relevance scores with high annotation agreement. State of the art models evaluated on our dataset show a significant gap to be closed in further work. Our dataset may be accessed here: https://github.com/iesl/CSFCube

==> figures/facetexamples.tex <==
\begin{table*}[t]
\caption{Examples of candidate papers similar along different facets
for the same query paper: A paper discussing compositional
vector-space models of negation can be similar along the topic of negation
or to compositional vector-space model based methods. A dataset paper
annotating data from
a hate speech forum is similar in background to other works tackling hate
speech, but methodologically similar to other articles generating datasets from
forums.}
\begin{tabular}{p{4.7cm}p{4.7cm}p{4.7cm}}
Query title &  Similar \texttt{background} candidate title  & Similar
\texttt{method}
candidate title
\\\hline\hline
 ``Not not bad'' is not ``bad'': A Distributional Account of Negation .
 &
Representing and Resolving Negation for Sentiment Analysis
& Mathematical Foundations for a Compositional Distributional Model of Meaning\\
Hate Speech Dataset from a White Supremacy Forum & Hierarchical CVAE for
Fine-Grained Hate Speech Classification
 & Measuring Online Affects in a White Supremacy Forum
    \end{tabular}
    \label{tab:facetexaamples}
    \end{table*}

==> figures/result-table.tex <==
\begin{table*}[t]
\caption{Test set results for the set of baselines methods. Metrics (R-Precision, Precision and Recall at 20, NDCG) are computed based on a 2-fold cross-validation. Superscripts for performance numbers indicate statistical significance with respect to a given method with Bonferroni corrections. Superscript on model names indicate reference for superscripts on the numbers. We only compute significance between models with superscripts for brevity. Letter superscripts indicate significance at $p=0.10$ and numbered superscripts indicate significance at $p=0.05$}.
\scalebox{0.8}{
\begin{tabular}{rcccc|cccc}
                     & \multicolumn{4}{c}{\texttt{background}}   & \multicolumn{4}{c}{\texttt{method}}        \\ 
                     & RP     & P@20   & R@20   & NDCG   & RP     & P@20   & R@20   & NDCG   \\\toprule
$^{1a}$\texttt{fabs\_tfidf}          & 0.2335 & 0.2719 & 0.458  & 0.7814 & 0.093  & 0.0983 & 0.3475 & 0.5787 \\
\texttt{fabs\_cbow200}        & 0.1961 & 0.1594 & 0.2797 & 0.6768 & 0.0865 & 0.0833 & 0.1569 & 0.5158 \\
\texttt{fabs\_tfidfcbow200}   & 0.1592 & 0.1687 & 0.2776 & 0.6977 & 0.0799 & 0.0601 & 0.1771 & 0.5187 \\
$^{2b}$\texttt{SentBERT-PP}              & 0.2124 & 0.2875 & 0.4667 & 0.7914 & 0.1000 & 0.1083 & 0.3630 & 0.595\\
\texttt{SentBERT-NLI}              & 0.1902 & 0.25 & 0.4013 & 0.758 & 0.0911 & 0.1146 & 0.289 & 0.5852\\
$^{3c}$SPECTER              & {0.2481} & \textbf{0.3531} & \textbf{0.5745} & {0.8224} & \textbf{0.1172} & {0.1358} & {0.4081} & {0.6277} \\
$^{4d}$SPECTER-ID              & \textbf{0.259} & 0.3406 & 0.5526 & \textbf{0.8348} & 0.0984 & \textbf{0.159} & \textbf{0.4316} & \textbf{0.6531}\\
\multicolumn{1}{l}{} & \multicolumn{4}{c}{\texttt{result}}       & \multicolumn{4}{c}{\texttt{all}}           \\ 
                     & RP     & P@20   & R@20   & NDCG   & RP     & P@20   & R@20   & NDCG   \\\toprule
$^{1a}$\texttt{fabs\_tfidf}          & 0.1135 & 0.1628 & 0.3857 & 0.6612 & 0.1459 & 0.1764 & 0.3969 & 0.6717 \\
\texttt{fabs\_cbow200}        & 0.1116 & 0.1042 & 0.2344 & 0.6022 & 0.1308 & 0.1147 & 0.2223 & 0.5964 \\
\texttt{fabs\_tfidfcbow200}   & 0.1043 & 0.1069 & 0.2439 & 0.6030  & 0.1138 & 0.1109 & 0.2313 & 0.6042 \\
$^{2b}$\texttt{SentBERT-PP}              & 0.136 & 0.1983 & 0.4173 & 0.719 & 0.1483 & 0.1962 & 0.4141 & 0.6998\\
\texttt{SentBERT-NLI}              & 0.1423 & 0.2205 & 0.4699 & 0.7213 & 0.1404 & 0.1942 & 0.3867 & 0.6868 \\
$^{3c}$SPECTER              & {0.1862} & {0.2378} & {0.5272} & {0.7547}$^1$ & \textbf{0.1829} & {0.2397} & {0.5014} & {0.7330}$^a$\\
$^{4d}$SPECTER-ID              & \textbf{0.1938}$^1$ & \textbf{0.2653}$^a$ & \textbf{0.6071}$^{ab}$ & \textbf{0.7789}$^1$ & 0.1825 & \textbf{0.2530}$^1$ & \textbf{0.5296}$^{1b}$ & \textbf{0.7541}$^{1b}$
\end{tabular}   
\label{tab-baseline-results}}
\end{table*}
